Step-by-Step Reasoning to Solve Grid Puzzles: Where do LLMs Falter?

Solving grid puzzles involves a significant amount of logical reasoning. Hence, it is a good domain to evaluate the reasoning capability of a model which can then guide us to improve the reasoning ability of models. However, most existing works evaluate only the final predicted answer of a puzzle, without delving into an in-depth analysis of the LLMs' reasoning chains (such as where they falter) or providing any finer metrics to evaluate them. Since LLMs may rely on simple heuristics or artifacts to predict the final answer, it is crucial to evaluate the generated reasoning chain beyond overall correctness measures, for accurately evaluating the reasoning abilities of LLMs. To this end, we first develop GridPuzzle, an evaluation dataset comprising 274 grid-based puzzles with different complexities. Second, we propose a new error taxonomy derived from manual analysis of reasoning chains from LLMs including GPT-4, Claude-3, Gemini, Mistral, and Llama-2. Then, we develop an LLM-based framework for large-scale subjective evaluation (i.e., identifying errors) and an objective metric, PuzzleEval, to evaluate the correctness of reasoning chains. Evaluating reasoning chains from LLMs leads to several interesting findings. We further show that existing prompting methods used for enhancing models' reasoning abilities do not improve performance on GridPuzzle. This highlights the importance of understanding fine-grained errors and presents a challenge for future research to enhance LLMs' puzzle-solving abilities by developing methods that address these errors. Data and source code are available at https://github.com/Mihir3009/GridPuzzle.

==> tables/sub_categories.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|p{8cm}}
\toprule
\textbf{Category}                                                                            & \textbf{Source}                                                                                                                                                      & \textbf{Sub-Category}                   & \textbf{Description}                                                                                                                                                                                                     \\ \midrule
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}Wrong Premise\\ or \\ No Conclusion\end{tabular}} & \multirow{6}{*}{From the clues (Example: From clue 4,....)}                                                                                                          & \multirow{2}{*}{Hallucination}          & When some information is completely out of context (e.g.,  objects/names/times), and not even present in clues                                                                                          \\
                                                                                             &                                                                                                                                                                      &                                         &                                                                                                                                                                                                                          \\ \cmidrule{3-4} 
                                                                                             &                                                                                                                                                                      & \multirow{2}{*}{Incomplete Information} & When to make a particular conclusion all the information is not present                                                                                                                                 \\
                                                                                             &                                                                                                                                                                      &                                         &                                                                                                                                                                                                                          \\ \cmidrule{3-4} 
                                                                                             &                                                                                                                                                                      & \multirow{2}{*}{Assumptions}            & When there are statements that are not derived conclusions and also not given in clues directly; can also be of the form “Let’s assume” (information present in this statement is relevant to the clue) \\
                                                                                             &                                                                                                                                                                      &                                         &                                                                                                                                                                                                                          \\ \cmidrule{2-4} 
                                                                                             & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Derived Conclusions using clues given in puzzle. \\ This information was not inherently given in the clues.\end{tabular}} & Error Propagation                       & When this premise is derived from a previous wrong conclusion                                                                                                                                                            \\ \cmidrule{3-4} 
                                                                                             &                                                                                                                                                                      & Incomplete Information                  & When to make a particular conclusion all the information is not present                                                                                                                                                  \\ \cmidrule{3-4} 
                                                                                             &                                                                                                                                                                      & Wrong Assumption                        & When the derived assumption is incorrect                                                                                                                                                                                 \\ \midrule
\multirow{3}{*}{Wrong Conclusion}                                                            & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Derived using the premise \\ (which itself is either taken \\ directly from the clues or derived)\end{tabular}}           & Wrong Reasoning                         & When the reasoning is wrong given whatever premise; the premise, in this case, can be both right or wrong                                                                                                                \\ \cline{3-4} 
                                                                                             &                                                                                                                                                                      & Error propagation                       & When the conclusion is wrong strictly because of the error in the premise; in this case, the premise is always wrong                                                                                                     \\ \cmidrule{3-4} 
                                                                                             &                                                                                                                                                                      & Wrong Elimination                       & When all information (premises) is present, but the model fails to make all possible conclusions                                                                                                                         \\ \bottomrule
\end{tabular}
}
\caption{List of sub-categories based on manual analysis.}
\end{table*}
